Utterance-level Aggregation For Speaker Recognition In The Wild

The objective of this paper is speaker recognition "in the wild"-where utterances may be of variable length and also contain irrelevant signals. Crucial elements in the design of deep networks for this task are the type of trunk (frame level) network, and the method of temporal aggregation. We propose a powerful speaker recognition deep network, using a "thin-ResNet" trunk architecture, and a dictionary-based NetVLAD or GhostVLAD layer to aggregate features across time, that can be trained end-to-end. We show that our network achieves state of the art performance by a significant margin on the VoxCeleb1 test set for speaker recognition, whilst requiring fewer parameters than previous methods. We also investigate the effect of utterance length on performance, and conclude that for "in the wild" data, a longer length is beneficial.

==> voxceleb1_ver2.tex <==

\begin{table*}[htb]
\footnotesize
\begin{center}
\begin{tabular}{l|l|c|c|c|c|c}
\hline
 & Front-end model & Loss & Dims & Aggregation & Training set & EER (\%)\\
\hline
\hline 
{\bf VoxCeleb1 test set} \\
\hline
Nagrani \etal \cite{Nagrani17} & I-vectors + PLDA& -- &-- &-- & VoxCeleb1 & 8.8\\
Nagrani \etal \cite{Nagrani17} & VGG-M & Softmax & 1024 & TAP & VoxCeleb1 & 10.2\\
\hline
Cai \etal \cite{cai2018exploring} & ResNet-34 & A-Softmax + PLDA & 128 & TAP &VoxCeleb1 & 4.46 \\
Cai \etal \cite{cai2018exploring} & ResNet-34 & A-Softmax + PLDA & 128 & SAP &VoxCeleb1 & 4.40 \\
Cai \etal \cite{cai2018exploring} & ResNet-34 & A-Softmax + PLDA & 128 & LDE &VoxCeleb1 & 4.48 \\
\hline
Okabe \etal \cite{okabe2018attentive} & TDNN (x-vector) & Softmax & 1500 & TAP &VoxCeleb1 & 4.70 \\
Okabe \etal \cite{okabe2018attentive} & TDNN (x-vector) & Softmax & 1500 & SAP &VoxCeleb1 & 4.19 \\
Okabe \etal \cite{okabe2018attentive} & TDNN (x-vector) & Softmax & 1500 & ASP &VoxCeleb1 & 3.85 \\
\hline
Hajibabaei \etal \cite{hajibabaei2018unified} & ResNet-20 & A-Softmax & 128 & TAP & VoxCeleb1 & 4.40 \\
Hajibabaei \etal \cite{hajibabaei2018unified} & ResNet-20 & AM-Softmax & 128 & TAP & VoxCeleb1 & 4.30 \\
\hline
Chung \etal \cite{Chung18a} & ResNet-34 & Softmax + Contrastive& 512 &TAP &VoxCeleb2 & 5.04 \\
Chung \etal \cite{Chung18a} & ResNet-50 & Softmax + Contrastive & 512 &TAP & VoxCeleb2 & 4.19 \\
\hline
{\bf Ours} & Thin ResNet-34 & Softmax& 512 &TAP & VoxCeleb2 & 10.48 \\
{\bf Ours} & Thin ResNet-34 & Softmax& 512 &NetVLAD & VoxCeleb2 & 3.57 \\
{\bf Ours} & Thin ResNet-34 & AM-Softmax & 512 &NetVLAD& VoxCeleb2 & 3.32 \\ 
{\bf Ours} & Thin ResNet-34 & Softmax& 512 &GhostVLAD & VoxCeleb2 &  \textbf{3.22} \\
{\bf Ours} & Thin ResNet-34 & AM-Softmax& 512 &GhostVLAD & VoxCeleb2 & 3.23 \\
%{\bf Ours (cleaned $\dagger$) } & Thin ResNet-34 & Softmax& 512 &GhostVLAD & VoxCeleb2 &  3.24 \\
%{\bf Ours} & Thin ResNet-34 & AM-Softmax& 512 &GhostVLAD & VoxCeleb2 & TRAINING \\
\hline
\hline  
{\bf VoxCeleb1-EC} \\ 
\hline 
Chung \etal \cite{Chung18a} & ResNet-50 & Softmax + Contrastive & 512 &TAP & VoxCeleb2 & 4.32 \\
%{\bf Ours} & Thin ResNet-34 & AM-Softmax & 512 & NetVLAD& VoxCeleb2 & 3.41 \\ 
%{\bf Ours} & Thin ResNet-34 & Softmax & 512 & GhostVLAD& VoxCeleb2 & \textbf{3.24} \\ 
{\bf Ours (cleaned $\dagger$) } & Thin ResNet-34 & Softmax & 512 & GhostVLAD& VoxCeleb2 & \textbf{3.13} \\ 
\hline
\hline 
{\bf VoxCeleb1-HC} \\ 
\hline 
Chung \etal \cite{Chung18a} & ResNet-50 & Softmax + Contrastive & 512 &TAP & VoxCeleb2 & 7.22 \\
%{\bf Ours} & Thin ResNet-34 & AM-Softmax & 512 &NetVLAD& VoxCeleb2 & 5.58 \\ 
%{\bf Ours} & Thin ResNet-34 & Softmax & 512 &GhostVLAD& VoxCeleb2 & \textbf{5.17} \\ 
{\bf Ours (cleaned $\dagger$) } & Thin ResNet-34 & Softmax & 512 &GhostVLAD& VoxCeleb2 & \textbf{5.06} \\ 
\hline
\end{tabular}
\end{center}
\vspace{-12pt}
\caption{Results for verification on the original VoxCeleb1
test set~\cite{Nagrani17} and the extended and hard
test sets (VoxCeleb-E and VoxCeleb-H)~\cite{Chung18a}. 
\cite{cai2018exploring,okabe2018attentive,hajibabaei2018unified} do not report results on the VoxCeleb1-EC and VoxCeleb1-HC)~\cite{Chung18a} test sets. {\bf TAP}: Temporal Average Pooling. {\bf SAP}: Self-attentive Pooling Layer~\cite{cai2018exploring}.} 
\label{tab:voxceleb1_verification}
\normalsize
\end{table*}
\normalsize

